Splicing positroid varieties

We construct an explicit isomorphism between an open subset in the open positroid variety $\Pi_{k,n}^{\circ}$ in the Grassmannian $\mathrm{Gr}(k,n)$ and the product of two open positroid varieties $\Pi_{k,n-a+1}^{\circ}\times \Pi_{k,a+k-1}^{\circ}$. In the respective cluster structures, this isomorphism is given by freezing a certain subset of cluster variables and applying a cluster quasi-equivalence.

==> Figures/Sigma3,8.tex <==
% https://q.uiver.app/#q=WzAsMTYsWzAsMCwiXFx0ZXh0Y29sb3J7Ymx1ZX17Njc4fSJdLFsxLDEsIjU3OCJdLFsyLDEsIjQ3OCJdLFszLDEsIjM3OCJdLFs0LDEsIjI3OCJdLFs1LDEsIlxcdGV4dGNvbG9ye2JsdWV9ezE3OH0iXSxbMSwyLCI1NjgiXSxbMiwyLCI0NTgiXSxbMywyLCIzNDgiXSxbNCwyLCIyMzgiXSxbNSwyLCJcXHRleHRjb2xvcntibHVlfXsxMjh9Il0sWzEsMywiXFx0ZXh0Y29sb3J7Ymx1ZX17NTY3fSJdLFsyLDMsIlxcdGV4dGNvbG9ye2JsdWV9ezQ1Nn0iXSxbMywzLCJcXHRleHRjb2xvcntibHVlfXszNDV9Il0sWzQsMywiXFx0ZXh0Y29sb3J7Ymx1ZX17MjM0fSJdLFs1LDMsIlxcdGV4dGNvbG9ye2JsdWV9ezEyM30iXSxbMCwxXSxbMSwyXSxbMiwzXSxbMyw0XSxbNCw1XSxbMSw2XSxbMiw3XSxbMyw4XSxbNCw5XSxbMTAsNF0sWzksM10sWzgsMl0sWzcsMV0sWzYsN10sWzcsOF0sWzgsOV0sWzksMTBdLFsxNSw5XSxbOCwxM10sWzksMTRdLFsxNCw4XSxbMTMsN10sWzcsMTJdLFsxMiw2XSxbNiwxMV1d
\begin{tikzcd}
	{\textcolor{blue}{678}} \\
	& 578 & 478 & 378 & 278 & {\textcolor{blue}{178}} \\
	& 568 & 458 & 348 & 238 & {\textcolor{blue}{128}} \\
	& {\textcolor{blue}{567}} & {\textcolor{blue}{456}} & {\textcolor{blue}{345}} & {\textcolor{blue}{234}} & {\textcolor{blue}{123}}
	\arrow[from=1-1, to=2-2]
	\arrow[from=2-2, to=2-3]
	\arrow[from=2-3, to=2-4]
	\arrow[from=2-4, to=2-5]
	\arrow[from=2-5, to=2-6]
	\arrow[from=2-2, to=3-2]
	\arrow[from=2-3, to=3-3]
	\arrow[from=2-4, to=3-4]
	\arrow[from=2-5, to=3-5]
	\arrow[from=3-6, to=2-5]
	\arrow[from=3-5, to=2-4]
	\arrow[from=3-4, to=2-3]
	\arrow[from=3-3, to=2-2]
	\arrow[from=3-2, to=3-3]
	\arrow[from=3-3, to=3-4]
	\arrow[from=3-4, to=3-5]
	\arrow[from=3-5, to=3-6]
	\arrow[from=4-6, to=3-5]
	\arrow[from=3-4, to=4-4]
	\arrow[from=3-5, to=4-5]
	\arrow[from=4-5, to=3-4]
	\arrow[from=4-4, to=3-3]
	\arrow[from=3-3, to=4-3]
	\arrow[from=4-3, to=3-2]
	\arrow[from=3-2, to=4-2]
\end{tikzcd}
